MorphBPE: A Morpho-Aware Tokenizer Bridging Linguistic Complexity for Efficient LLM Training Across Morphologies

Tokenization is fundamental to Natural Language Processing (NLP), directly impacting model efficiency and linguistic fidelity. While Byte Pair Encoding (BPE) is widely used in Large Language Models (LLMs), it often disregards morpheme boundaries, leading to suboptimal segmentation, particularly in morphologically rich languages. We introduce MorphBPE, a morphology-aware extension of BPE that integrates linguistic structure into subword tokenization while preserving statistical efficiency. Additionally, we propose two morphology-based evaluation metrics: (i) Morphological Consistency F1-Score, which quantifies the consistency between morpheme sharing and token sharing, contributing to LLM training convergence, and (ii) Morphological Edit Distance, which measures alignment between morphemes and tokens concerning interpretability. Experiments on English, Russian, Hungarian, and Arabic across 300M and 1B parameter LLMs demonstrate that MorphBPE consistently reduces cross-entropy loss, accelerates convergence, and improves morphological alignment scores. Fully compatible with existing LLM pipelines, MorphBPE requires minimal modifications for integration. The MorphBPE codebase and tokenizer playground will be available at: https://github.com/llm-lab-org/MorphBPE and https://tokenizer.llm-lab.org

==> backup.tex <==

%\begin{table}
%\centering
%\caption{LLM Training Parameters for Evaluating $MorphBPE$ vs. BPE Across Languages with Diverse Morphologies: Hungarian, Arabic, Russian, and English.}
%\label{tab:llm_params}
%\resizebox{0.8\width}{!}{%
%\begin{tabular}{lccc}
%\toprule
% Language &         \# of Tokens (Model: 300M) &  \# of Tokens (Model: 1B) &  Token Vocab. Size \\
%\midrule
%Hungarian &                 6B &            20B &                  24K \\
%  Russian &                6B &            20B &                  64K \\
%  English &                6B &            20B &                  96K \\
%   Arabic &         6B &            20B &                  96K \\
%\bottomrule
%\end{tabular}%
%}
%\end{table}


%\begin{table*}[ht!]
%  \centering
%    \label{tab:metrics}
%    \caption{Intrinsic valuation metrics proposed for the evaluation of tokenizers and their definitions.}
%  \resizebox{0.75\width}{!}{\begin{tabular}{lll}
%        \toprule
%        \textbf{Metric} & \textbf{Symbol} & \textbf{Definition} \\
%        \midrule
%        Fertility & \(\phi\) & \( \phi = \frac{\text{Number of tokenizer-generated tokens}}{\text{Number of whitespace-based tokens}} \) \\
%        Morphology Edit Distance Score & \(\mu\) & Pairwise alignment score measuring tokenization consistency with morphological segmentation \\
%        Perplexity & \(\pi\) & \( \pi = \exp \left( -\frac{1}{N} \sum_{i=1}^{N} \log P(w_i) \right) \), where \( P(w_i) \) is the model's probability of word \( w_i \) \\
%        \bottomrule
%    \end{tabular}}
%\end{table*}


% \begin{table*}[ht!]
%   \centering
%     \label{tab:metrics}
%     \caption{Intrinsic valuation metrics proposed for the evaluation of tokenizers and their definitions.}
%   \resizebox{0.75\width}{!}{\begin{tabular}{lll}
%         \toprule
%         \textbf{Metric} & \textbf{Symbol} & \textbf{Definition} \\
%         \midrule
%         Fertility & \(\phi\) & \( \phi = \frac{\text{Number of tokenizer-generated tokens}}{\text{Number of whitespace-based tokens}} \) \\
%         Morphology Edit Distance Score & \(\mu\) & Pairwise alignment score measuring tokenization consistency with morphological segmentation \\
%         Perplexity & \(\pi\) & \( \pi = \exp \left( -\frac{1}{N} \sum_{i=1}^{N} \log P(w_i) \right) \), where \( P(w_i) \) is the model's probability of word \( w_i \) \\
%         \bottomrule
%     \end{tabular}}
% \end{table*}

% \begin{figure*}[ht!]
%     \centering
%     \includegraphics[width=0.95\textwidth]{diagrams/ce_loss_log.pdf}
%     \caption{Comparison of training cross-entropy loss between BPE and $MorphBPE$ across four languages. Results are shown for both the small (300M) and large (1B) models.}
%     \label{fig:cross_entropy_loss}
% \end{figure*}


    % \item \textbf{Fertility rate aligns with morphological complexity}: For English, which has relatively simple morphology, both BPE and $MorphBPE$ show **higher fertility rates** compared to **Hungarian and Russian**. However, the fertility gap between $MorphBPE$ and BPE is **larger in languages with complex morphology**, indicating that $MorphBPE$ generates **more interpretable** tokenization with better morpheme segmentation.

%\item \textbf{BPE over-segments morphologically rich languages}: As seen in **Figure~\ref{fig:morph_fertility}**, BPE produces **significantly higher morphological distance** in **Hungarian and Arabic**, reinforcing the intuition that it fails to respect meaningful morpheme boundaries. In contrast, $MorphBPE$ mitigates this issue by aligning better with the underlying linguistic structure.

%\item \textbf{Computational implications}: The fertility rate differences suggest that BPE might lead to inefficient tokenization, increasing sequence lengths unnecessarily. This can **negatively impact training and inference efficiency** in LLMs, especially for morphologically rich languages.
